Contaminated Multivariate Time-Series Anomaly Detection with Spatio-Temporal Graph Conditional Diffusion Models

Mainstream unsupervised anomaly detection algorithms often excel in academic datasets, yet their real-world performance is restricted due to the controlled experimental conditions involving clean training data. Addressing the challenge of training with noise, a prevalent issue in practical anomaly detection, is frequently overlooked. In a pioneering endeavor, this study delves into the realm of label-level noise within sensory time-series anomaly detection (TSAD). This paper presents a novel and practical end-to-end unsupervised TSAD when the training data is contaminated with anomalies. The introduced approach, called TSAD-C, is devoid of access to abnormality labels during the training phase. TSAD-C encompasses three core modules: a Decontaminator to rectify anomalies (aka noise) present during training, a Long-range Variable Dependency Modeling module to capture long-term intra- and inter-variable dependencies within the decontaminated data that is considered as a surrogate of the pure normal data, and an Anomaly Scoring module to detect anomalies from all types. Our extensive experiments conducted on four reliable and diverse datasets conclusively demonstrate that TSAD-C surpasses existing methodologies, thus establishing a new state-of-the-art in the TSAD field.

==> refs.tex <==
@article{james2004independent,
  title={Independent component analysis for biomedical signals},
  author={James, Christopher J and Hesse, Christian W},
  journal={Physiological measurement},
  volume={26},
  number={1},
  pages={R15},
  year={2004},
  publisher={IOP Publishing}
}

@article{tao2005intracranial,
  title={Intracranial EEG substrates of scalp EEG interictal spikes},
  author={Tao, James X and Ray, Amit and Hawes-Ebersole, Susan and Ebersole, John S},
  journal={Epilepsia},
  volume={46},
  number={5},
  pages={669--676},
  year={2005},
  publisher={Wiley Online Library}
}

@article{berkaya2018survey,
  title={A survey on ECG analysis},
  author={Berkaya, Selcan Kaplan and Uysal, Alper Kursat and Gunal, Efnan Sora and Ergin, Semih and Gunal, Serkan and Gulmezoglu, M Bilginer},
  journal={Biomedical Signal Processing and Control},
  volume={43},
  pages={216--235},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{khalkhali2021low,
  title={Low Latency Real-Time Seizure Detection Using Transfer Deep Learning},
  author={Khalkhali, Vahid and Shawki, Nabila and Shah, Vinit and Golmohammadi, Meysam and Obeid, Iyad and Picone, Joseph},
  booktitle={2021 IEEE Signal Processing in Medicine and Biology Symposium (SPMB)},
  pages={1--7},
  year={2021},
  organization={IEEE}
}

@article{rashed2021deep,
  title={A deep convolutional neural network method to detect seizures and characteristic frequencies using epileptic electroencephalogram (EEG) data},
  author={Rashed-Al-Mahfuz, Md and Moni, Mohammad Ali and Uddin, Shahadat and Alyami, Salem A and Summers, Matthew A and Eapen, Valsamma},
  journal={IEEE Journal of Translational Engineering in Health and Medicine},
  volume={9},
  pages={1--12},
  year={2021},
  publisher={IEEE}
}

@article{thuwajit2021eegwavenet,
  title={EEGWaveNet: Multiscale CNN-Based Spatiotemporal Feature Extraction for EEG Seizure Detection},
  author={Thuwajit, Punnawish and Rangpong, Phurin and Sawangjai, Phattarapong and Autthasan, Phairot and Chaisaen, Rattanaphon and Banluesombatkul, Nannapas and Boonchit, Puttaranun and Tatsaringkansakul, Nattasate and Sudhawiyangkul, Thapanun and Wilaiprasitporn, Theerawit},
  journal={IEEE Transactions on Industrial Informatics},
  volume={18},
  number={8},
  pages={5547--5557},
  year={2021},
  publisher={IEEE}
}

@inproceedings{tang2021self,
  title={Self-Supervised Graph Neural Networks for Improved Electroencephalographic Seizure Analysis},
  author={Tang, Siyi and Dunnmon, Jared and Saab, Khaled Kamal and Zhang, Xuan and Huang, Qianying and Dubost, Florian and Rubin, Daniel and Lee-Messer, Christopher},
  booktitle={International Conference on Learning Representations},
  year={2021}
}

@inproceedings{ho2023self,
  title={Self-Supervised Learning for Anomalous Channel Detection in EEG Graphs: Application to Seizure Analysis},
  author={Ho, Thi Kieu Khanh and Armanfard, Narges},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={37},
  pages={7866--7874},
  year={2023}
}

@inproceedings{tang2023modeling,
  title={Modeling Multivariate Biosignals With Graph Neural Networks and Structured State Space Models},
  author={Tang, Siyi and Dunnmon, Jared A and Liangqiong, Qu and Saab, Khaled K and Baykaner, Tina and Lee-Messer, Christopher and Rubin, Daniel L},
  booktitle={Conference on Health, Inference, and Learning},
  pages={50--71},
  year={2023},
  organization={PMLR}
}

@article{loh2022automated,
  title={Automated detection of cyclic alternating pattern and classification of sleep stages using deep neural network},
  author={Loh, Hui Wen and Ooi, Chui Ping and Dhok, Shivani G and Sharma, Manish and Bhurane, Ankit A and Acharya, U Rajendra},
  journal={Applied Intelligence},
  volume={52},
  number={3},
  pages={2903--2917},
  year={2022},
  publisher={Springer}
}

@article{xu2022review,
  title={A review of automated sleep disorder detection},
  author={Xu, Shuting and Faust, Oliver and Silvia, Seoni and Chakraborty, Subrata and Barua, Prabal Datta and Loh, Hui Wen and Elphick, Heather and Molinari, Filippo and Acharya, U Rajendra},
  journal={Computers in Biology and Medicine},
  pages={106100},
  year={2022},
  publisher={Elsevier}
}

@article{ettahiri2022eeg,
  title={EEG brain signals to detect the sleep health of a driver: An automated framework system based on deep learning},
  author={Ettahiri, Halima and Ferr{\'a}ndez Vicente, Jos{\'e} Manuel and Fechtali, Taoufiq},
  journal={Frontiers in Human Neuroscience},
  volume={16},
  pages={915276},
  year={2022},
  publisher={Frontiers}
}


@article{isin2017cardiac,
  title={Cardiac arrhythmia detection using deep learning},
  author={Isin, Ali and Ozdalili, Selen},
  journal={Procedia computer science},
  volume={120},
  pages={268--275},
  year={2017},
  publisher={Elsevier}
}

@article{rath2021heart,
  title={Heart disease detection using deep learning methods from imbalanced ECG samples},
  author={Rath, Adyasha and Mishra, Debahuti and Panda, Ganapati and Satapathy, Suresh Chandra},
  journal={Biomedical Signal Processing and Control},
  volume={68},
  pages={102820},
  year={2021},
  publisher={Elsevier}
}

@article{abubaker2022detection,
  title={Detection of cardiovascular diseases in ECG images using machine learning and deep learning methods},
  author={Abubaker, Mohammed B and Babayi{\u{g}}it, Bilal},
  journal={IEEE Transactions on Artificial Intelligence},
  volume={4},
  number={2},
  pages={373--382},
  year={2022},
  publisher={IEEE}
}

@article{lim2021noisy,
  title={Noisy recurrent neural networks},
  author={Lim, Soon Hoe and Erichson, N Benjamin and Hodgkinson, Liam and Mahoney, Michael W},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={5124--5137},
  year={2021}
}

@inproceedings{katharopoulos2020transformers,
  title={Transformers are rnns: Fast autoregressive transformers with linear attention},
  author={Katharopoulos, Angelos and Vyas, Apoorv and Pappas, Nikolaos and Fleuret, Fran{\c{c}}ois},
  booktitle={International Conference on Machine Learning},
  pages={5156--5165},
  year={2020},
  organization={PMLR}
}

@article{strodthoff2020deep,
  title={Deep learning for ECG analysis: Benchmarks and insights from PTB-XL},
  author={Strodthoff, Nils and Wagner, Patrick and Schaeffter, Tobias and Samek, Wojciech},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={25},
  number={5},
  pages={1519--1528},
  year={2020},
  publisher={IEEE}
}

@inproceedings{pradhan2022hand,
  title={Hand gesture recognition and biometric authentication using a multi-day dataset},
  author={Pradhan, Ashirbad and He, Jiayuan and Jiang, Ning},
  booktitle={Intelligent Robotics and Applications: 15th International Conference, ICIRA 2022, Harbin, China, August 1--3, 2022, Proceedings, Part IV},
  pages={375--385},
  year={2022},
  organization={Springer}
}

@article{ho2023graph,
  title={Graph Anomaly Detection in Time Series: A Survey},
  author={Ho, Thi Kieu Khanh and Karami, Ali and Armanfard, Narges},
  journal={arXiv preprint arXiv:2302.00058},
  year={2023}
}

@inproceedings{gu2021efficiently,
  title={Efficiently modeling long sequences with structured state spaces},
  author={Gu, Albert and Goel and Karan and R{\'e}, Christopher},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

@article{morley201610,
  title={10-20 system EEG Placement},
  author={Morley, Andrew and Hill, Lizzie and Kaditis, AG},
  journal={European Respiratory Society, European Respiratory Society},
  year={2016}
}

@inproceedings{gao2022equivalence,
  title={On the equivalence between temporal and static equivariant graph representations},
  author={Gao, Jianfei and Ribeiro, Bruno},
  booktitle={International Conference on Machine Learning},
  pages={7052--7076},
  year={2022},
  organization={PMLR}
}

@article{alcaraz2022diffusion,
  title={Diffusion-based time series imputation and forecasting with structured state space models},
  author={Alcaraz, Juan Miguel Lopez and Strodthoff, Nils},
  journal={Transactions on Machine Learning Research},
  year={2022}
}

@inproceedings{khayati2020mind,
  title={Mind the gap: an experimental evaluation of imputation of missing values techniques in time series},
  author={Khayati, Mourad and Lerner, Alberto and Tymchenko, Zakhar and Cudr{\'e}-Mauroux, Philippe},
  booktitle={Proceedings of the VLDB Endowment},
  volume={13},
  pages={768--782},
  year={2020}
}

@inproceedings{sohl2015deep,
  title={Deep unsupervised learning using nonequilibrium thermodynamics},
  author={Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
  booktitle={International conference on machine learning},
  pages={2256--2265},
  year={2015},
  organization={PMLR}
}

@article{zhang2023diffusionad,
  title={DiffusionAD: Denoising Diffusion for Anomaly Detection},
  author={Zhang, Hui and Wang, Zheng and Wu, Zuxuan and Jiang, Yu-Gang},
  journal={arXiv preprint arXiv:2303.08730},
  year={2023}
}

@article{gu2020hippo,
  title={Hippo: Recurrent memory with optimal polynomial projections},
  author={Gu, Albert and Dao, Tri and Ermon, Stefano and Rudra, Atri and R{\'e}, Christopher},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1474--1487},
  year={2020}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{zhu2021survey,
  title={A survey on graph structure learning: Progress and opportunities},
  author={Zhu, Yanqiao and Xu, Weizhi and Zhang, Jinghao and Du, Yuanqi and Zhang, Jieyu and Liu, Qiang and Yang, Carl and Wu, Shu},
  booktitle={International Joint Conference on Artificial Intelligence},
  year={2022}
}

@inproceedings{xu2018powerful,
  title={How powerful are graph neural networks?},
  author={Xu, Keyulu and Hu, Weihua and Leskovec, Jure and Jegelka, Stefanie},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@article{liu2018open,
  title={An open access database for evaluating the algorithms of electrocardiogram rhythm and morphology abnormality detection},
  author={Liu, Feifei and Liu, Chengyu and Zhao, Lina and Zhang, Xiangyu and Wu, Xiaoling and Xu, Xiaoyan and Liu, Yulin and Ma, Caiyun and Wei, Shoushui and He, Zhiqiang and others},
  journal={Journal of Medical Imaging and Health Informatics},
  volume={8},
  number={7},
  pages={1368--1373},
  year={2018},
  publisher={American Scientific Publishers}
}

@article{guillot2020dreem,
  title={Dreem open datasets: Multi-scored sleep datasets to compare human and automated sleep staging},
  author={Guillot, Antoine and Sauvet, Fabien and During, Emmanuel H and Thorey, Valentin},
  journal={IEEE transactions on neural systems and rehabilitation engineering},
  volume={28},
  number={9},
  pages={1955--1965},
  year={2020},
  publisher={IEEE}
}

@article{shah2018temple,
  title={The temple university hospital seizure detection corpus},
  author={Shah, Vinit and Von Weltin, Eva and Lopez, Silvia and McHugh, James Riley and Veloso, Lillian and Golmohammadi, Meysam and Obeid, Iyad and Picone, Joseph},
  journal={Frontiers in neuroinformatics},
  volume={12},
  pages={83},
  year={2018},
  publisher={Frontiers Media SA}
}

@inproceedings{davis2006relationship,
  title={The relationship between Precision-Recall and ROC curves},
  author={Davis, Jesse and Goadrich, Mark},
  booktitle={Proceedings of the 23rd international conference on Machine learning},
  pages={233--240},
  year={2006}
}

@article{wang2018lstm,
  title={LSTM-based EEG classification in motor imagery tasks},
  author={Wang, Ping and Jiang, Aimin and Liu, Xiaofeng and Shang, Jing and Zhang, Li},
  journal={IEEE transactions on neural systems and rehabilitation engineering},
  volume={26},
  number={11},
  pages={2086--2095},
  year={2018},
  publisher={IEEE}
}

@inproceedings{jia2020graphsleepnet,
  title={GraphSleepNet: Adaptive Spatial-Temporal Graph Convolutional Networks for Sleep Stage Classification.},
  author={Jia, Ziyu and Lin, Youfang and Wang, Jing and Zhou, Ronghao and Ning, Xiaojun and He, Yuanlai and Zhao, Yaoshuai},
  booktitle={IJCAI},
  volume={2021},
  pages={1324--1330},
  year={2020}
}

@article{wei2023lstm,
  title={LSTM-autoencoder-based anomaly detection for indoor air quality time-series data},
  author={Wei, Yuanyuan and Jang-Jaccard, Julian and Xu, Wen and Sabrina, Fariza and Camtepe, Seyit and Boulic, Mikael},
  journal={IEEE Sensors Journal},
  volume={23},
  number={4},
  pages={3787--3800},
  year={2023},
  publisher={IEEE}
}

@article{du2022graph,
  title={Graph autoencoder-based unsupervised outlier detection},
  author={Du, Xusheng and Yu, Jiong and Chu, Zheng and Jin, Lina and Chen, Jiaying},
  journal={Information Sciences},
  volume={608},
  pages={532--550},
  year={2022},
  publisher={Elsevier}
}

@article{jiang2022softpatch,
  title={Softpatch: Unsupervised anomaly detection with noisy data},
  author={Jiang, Xi and Liu, Jianlin and Wang, Jinbao and Nie, Qiang and Wu, Kai and Liu, Yong and Wang, Chengjie and Zheng, Feng},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={15433--15445},
  year={2022}
}

@inproceedings{thodoroff2016learning,
  title={Learning robust features using deep learning for automatic seizure detection},
  author={Thodoroff, Pierre and Pineau, Joelle and Lim, Andrew},
  booktitle={Machine learning for healthcare conference},
  pages={178--190},
  year={2016},
  organization={PMLR}
}

@inproceedings{deng2021graph,
  title={Graph neural network-based anomaly detection in multivariate time series},
  author={Deng, Ailin and Hooi, Bryan},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  pages={4027--4035},
  year={2021}
}

@inproceedings{chen2022deep,
  title={Deep variational graph convolutional recurrent network for multivariate time series anomaly detection},
  author={Chen, Wenchao and Tian, Long and Chen, Bo and Dai, Liang and Duan, Zhibin and Zhou, Mingyuan},
  booktitle={International Conference on Machine Learning},
  pages={3621--3633},
  year={2022},
  organization={PMLR}
}

@inproceedings{carmona2022neural,
  title={Neural contextual anomaly detection for time series},
  author={Carmona, Chris U and Aubet, Fran{\c{c}}ois-Xavier and Flunkert, Valentin and Gasthaus, Jan},
   booktitle={International Joint Conference on Artificial Intelligence},
  year={2022}
}

@inproceedings{lai2023open,
  title={Open-Set Multivariate Time-Series Anomaly Detection},
  author={Lai, Thomas and Ho, Thi Kieu Khanh and Armanfard, Narges},
  booktitle={European Conference on Artificial Intelligence},
  year={2024}
}

@article{kuan2017quantile,
  title={Quantile regression on quantile ranges--A threshold approach},
  author={Kuan, Chung-Ming and Michalopoulos and Christos and Xiao, Zhijie},
  journal={Journal of Time Series Analysis},
  volume={38},
  number={1},
  pages={99--119},
  year={2017},
  publisher={Wiley Online Library}
}

@inproceedings{su2019robust,
  title={Robust anomaly detection for multivariate time series through stochastic recurrent neural network},
  author={Su, Ya and Zhao, Youjian and Niu, Chenhao and Liu, Rong and Sun, Wei and Pei, Dan},
  booktitle={Proceedings of the 25th ACM SIGKDD international conference on knowledge discovery \& data mining},
  pages={2828--2837},
  year={2019}
}

@article{wagner2023timesead,
  title={TimeseAD: Benchmarking deep multivariate time-series anomaly detection},
  author={Wagner, Dennis and Michels, Tobias and Schulz, Florian CF and Nair, Arjun and Rudolph, Maja and Kloft, Marius},
  journal={Transactions on Machine Learning Research},
  year={2023}
}

@article{wu2021current,
  title={Current time series anomaly detection benchmarks are flawed and are creating the illusion of progress},
  author={Wu, Renjie and Keogh, Eamonn},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2021},
  publisher={IEEE}
}

@inproceedings{li2021multivariate,
  title={Multivariate time series anomaly detection and interpretation using hierarchical inter-metric and temporal embedding},
  author={Li, Zhihan and Zhao, Youjian and Han, Jiaqi and Su, Ya and Jiao, Rui and Wen, Xidao and Pei, Dan},
  booktitle={Proceedings of the 27th ACM SIGKDD conference on knowledge discovery \& data mining},
  pages={3220--3230},
  year={2021}
}

@inproceedings{hojjati2023multivariate,
  title={Multivariate time-series anomaly detection with temporal self-supervision and graphs: Application to vehicle failure prediction},
  author={Hojjati, Hadi and Sadeghi, Mohammadreza and Armanfard, Narges},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={242--259},
  year={2023},
  organization={Springer}
}

@article{shen2020timeseries,
  title={Timeseries anomaly detection using temporal hierarchical one-class network},
  author={Shen, Lifeng and Li, Zhuocong and Kwok, James},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={13016--13026},
  year={2020}
}

@inproceedings{loshchilov2017decoupled,
  title={Decoupled weight decay regularization},
  author={Loshchilov, Ilya and Hutter, Frank},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{loshchilov2016sgdr,
  title={Sgdr: Stochastic gradient descent with warm restarts},
  author={loshchilov, Ilya and Hutter, Frank},
  booktitle={International Conference on Learning Representations},
  year={2017}
}

@inproceedings{audibert2020usad,
  title={Usad: Unsupervised anomaly detection on multivariate time series},
  author={Audibert, Julien and Michiardi, Pietro and Guyard, Fr{\'e}d{\'e}ric and Marti, S{\'e}bastien and Zuluaga, Maria A},
  booktitle={Proceedings of the 26th ACM SIGKDD international conference on knowledge discovery \& data mining},
  pages={3395--3404},
  year={2020}
}

@inproceedings{yang2023dcdetector,
  title={Dcdetector: Dual attention contrastive representation learning for time series anomaly detection},
  author={Yang, Yiyuan and Zhang, Chaoli and Zhou, Tian and Wen, Qingsong and Sun, Liang},
  booktitle={Proceedings of the 29th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={3033--3045},
  year={2023}
}


@article{chen2024imdiffusion,
  title={Imdiffusion: Imputed diffusion models for multivariate time series anomaly detection},
  author={Chen, Yuhang and Zhang, Chaoyun and Ma, Minghua and Liu, Yudong and Ding, Ruomeng and Li, Bowen and He, Shilin and Rajmohan, Saravan and Lin, Qingwei and Zhang, Dongmei},
  journal={Proceedings of the VLDB Endowment},
  year={2024},
}

@article{schmidl2022anomaly,
  title={Anomaly detection in time series: a comprehensive evaluation},
  author={Schmidl, Sebastian and Wenig, Phillip and Papenbrock, Thorsten},
  journal={Proceedings of the VLDB Endowment},
  volume={15},
  number={9},
  pages={1779--1797},
  year={2022},
}

@inproceedings{kim2022towards,
  title={Towards a rigorous evaluation of time-series anomaly detection},
  author={Kim, Siwon and Choi, Kukjin and Choi, Hyun-Soo and Lee, Byunghan and Yoon, Sungroh},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={7194--7201},
  year={2022}
}

@article{croitoru2023diffusion,
  title={Diffusion models in vision: A survey},
  author={Croitoru, Florinel-Alin and Hondru, Vlad and Ionescu, Radu Tudor and Shah, Mubarak},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={45},
  number={9},
  pages={10850--10869},
  year={2023},
  publisher={IEEE}
}

@inproceedings{sun2024unraveling,
  title={Unraveling the ‘Anomaly’in time series anomaly detection: a self-supervised tri-domain solution},
  author={Sun, Yuting and Pang, Guansong and Ye, Guanhua and Chen, Tong and Hu, Xia and Yin, Hongzhi},
  booktitle={2024 IEEE 40th International Conference on Data Engineering (ICDE)},
  pages={981--994},
  year={2024},
  organization={IEEE}
}

@inproceedings{fang2024temporal,
  title={Temporal-Frequency Masked Autoencoders for Time Series Anomaly Detection},
  author={Fang, Yuchen and Xie, Jiandong and Zhao, Yan and Chen, Lu and Gao, Yunjun and Zheng, Kai},
  booktitle={2024 IEEE 40th International Conference on Data Engineering (ICDE)},
  pages={1228--1241},
  year={2024},
  organization={IEEE}
}

@article{zamanzadeh2022deep,
  title={Deep learning for time series anomaly detection: A survey},
  author={Zamanzadeh Darban, Zahra and Webb, Geoffrey I and Pan, Shirui and Aggarwal, Charu and Salehi, Mahsa},
  journal={ACM Computing Surveys},
  year={2022},
  publisher={ACM New York, NY}
}

@article{blazquez2021review,
  title={A review on outlier/anomaly detection in time series data},
  author={Bl{\'a}zquez-Garc{\'\i}a, Ane and Conde, Angel and Mori, Usue and Lozano, Jose A},
  journal={ACM computing surveys (CSUR)},
  volume={54},
  number={3},
  pages={1--33},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{ding2022catching,
  title={Catching both gray and black swans: Open-set supervised anomaly detection},
  author={Ding, Choubo and Pang, Guansong and Shen, Chunhua},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={7388--7398},
  year={2022}
}

@inproceedings{tian2022anomaly,
  title={Anomaly detection by leveraging incomplete anomalous knowledge with anomaly-aware bidirectional gans},
  author={Tian, Bowen and Su, Qinliang and Yin, Jian},
  booktitle={Proceedings of the Thirty-First International Joint Conference on Artificial Intelligence},
  year={2022}
}

@article{liang2021consistent,
  title={Consistent Anomaly Detection and Localization of Multivariate Time Series via Cross-Correlation Graph-Based Encoder--Decoder GAN},
  author={Liang, Haoran and Song, Lei and Du, Junrong and Li, Xuzhi and Guo, Lili},
  journal={IEEE Transactions on Instrumentation and Measurement},
  volume={71},
  pages={1--10},
  year={2021},
  publisher={IEEE}
}

@article{deng2022graph,
  title={Graph convolutional adversarial networks for spatiotemporal anomaly detection},
  author={Deng, Leyan and Lian, Defu and Huang, Zhenya and Chen, Enhong},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={33},
  number={6},
  pages={2416--2428},
  year={2022},
  publisher={IEEE}
}

@inproceedings{han2022learning,
  title={Learning Sparse Latent Graph Representations for Anomaly Detection in Multivariate Time Series},
  author={Han, Siho and Woo, Simon S},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={2977--2986},
  year={2022}
}

@inproceedings{zhao2020multivariate,
  title={Multivariate time-series anomaly detection via graph attention network},
  author={Zhao, Hang and Wang, Yujing and Duan, Juanyong and Huang, Congrui and Cao, Defu and Tong, Yunhai and Xu, Bixiong and Bai, Jing and Tong, Jie and Zhang, Qi},
  booktitle={IEEE International Conference on Data Mining},
  pages={841--850},
  year={2020},
}

@inproceedings{dai2022graph,
  title={Graph-Augmented Normalizing Flows for Anomaly Detection of Multiple Time Series},
  author={Dai, Enyan and Chen, Jie},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

@inproceedings{goel2022s,
  title={It’s raw! audio generation with state-space models},
  author={Goel, Karan and Gu, Albert and Donahue, Chris and R{\'e}, Christopher},
  booktitle={International Conference on Machine Learning},
  pages={7616--7633},
  year={2022},
  organization={PMLR}
}

@article{tay2020long,
  title={Long range arena: A benchmark for efficient transformers},
  author={Tay, Yi and Dehghani, Mostafa and Abnar, Samira and Shen, Yikang and Bahri, Dara and Pham, Philip and Rao, Jinfeng and Yang, Liu and Ruder, Sebastian and Metzler, Donald},
  journal={arXiv preprint arXiv:2011.04006},
  year={2020}
}

@inproceedings{flaborea2023multimodal,
  title={Multimodal motion conditioned diffusion model for skeleton-based video anomaly detection},
  author={Flaborea, Alessandro and Collorone, Luca and Di Melendugno, Guido Maria D'Amely and D'Arrigo, Stefano and Prenkaj, Bardh and Galasso, Fabio},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={10318--10329},
  year={2023}
}

@inproceedings{karami2024graph,
  title={Graph-Jigsaw Conditioned Diffusion Model for Skeleton-based Video Anomaly Detection},
  author={Karami, Ali and Ho, Thi Kieu Khanh and Armanfard, Narges},
  booktitle={EEE/CVF Winter Conference on Applications of Computer Vision},
  year={2025}
}

@article{tashiro2021csdi,
  title={Csdi: Conditional score-based diffusion models for probabilistic time series imputation},
  author={Tashiro, Yusuke and Song, Jiaming and Song, Yang and Ermon, Stefano},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={24804--24816},
  year={2021}
}

@inproceedings{rasul2021autoregressive,
  title={Autoregressive denoising diffusion models for multivariate probabilistic time series forecasting},
  author={Rasul, Kashif and Seward, Calvin and Schuster, Ingmar and Vollgraf, Roland},
  booktitle={International Conference on Machine Learning},
  pages={8857--8868},
  year={2021},
  organization={PMLR}
}

@inproceedings{livernoche2023diffusion,
  title={On diffusion modeling for anomaly detection},
  author={Livernoche, Victor and Jain, Vineet and Hezaveh, Yashar and Ravanbakhsh, Siamak},
  booktitle={International Conference on Learning Representations},
  year={2024},
}

@inproceedings{wolleb2022diffusion,
  title={Diffusion models for medical anomaly detection},
  author={Wolleb, Julia and Bieder, Florentin and Sandk{\"u}hler, Robin and Cattin, Philippe C},
  booktitle={International Conference on Medical image computing and computer-assisted intervention},
  pages={35--45},
  year={2022},
  organization={Springer}
}

@misc{laptev2015s5,
  title={S5-A labeled anomaly detection dataset, version 1.0 (16M)},
  author={Laptev, N and Amizadeh, S and Billawala, Y},
  year={2015},
  publisher={Mar}
}

@inproceedings{hundman2018detecting,
  title={Detecting spacecraft anomalies using lstms and nonparametric dynamic thresholding},
  author={Hundman, Kyle and Constantinou, Valentino and Laporte, Christopher and Colwell, Ian and Soderstrom, Tom},
  booktitle={Proceedings of the 24th ACM SIGKDD international conference on knowledge discovery \& data mining},
  pages={387--395},
  year={2018}
}

@inproceedings{mathur2016swat,
  title={SWaT: A water treatment testbed for research and training on ICS security},
  author={Mathur, Aditya P and Tippenhauer, Nils Ole},
  booktitle={2016 international workshop on cyber-physical systems for smart water networks (CySWater)},
  pages={31--36},
  year={2016},
  organization={IEEE}
}

@inproceedings{ahmed2017wadi,
  title={WADI: a water distribution testbed for research in the design of secure cyber physical systems},
  author={Ahmed, Chuadhry Mujeeb and Palleti, Venkata Reddy and Mathur, Aditya P},
  booktitle={Proceedings of the 3rd international workshop on cyber-physical systems for smart water networks},
  pages={25--28},
  year={2017}
}

@inproceedings{wang2024fully,
  title={Fully-Connected Spatial-Temporal Graph for Multivariate Time-Series Data},
  author={Wang, Yucheng and Xu, Yuecong and Yang, Jianfei and Wu, Min and Li, Xiaoli and Xie, Lihua and Chen, Zhenghua},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={38},
  number={14},
  pages={15715--15724},
  year={2024}
}

